Smart Fitting Room: A One-stop Framework for Matching-aware Virtual Try-on

The development of virtual try-on has revolutionized online shopping by allowing customers to visualize themselves in various fashion items, thus extending the in-store try-on experience to the cyber space. Although virtual try-on has attracted considerable research initiatives, existing systems only focus on the quality of image generation, overlooking whether the fashion item is a good match to the given person and clothes. Recognizing this gap, we propose to design a one-stop Smart Fitting Room, with the novel formulation of matching-aware virtual try-on. Following this formulation, we design a Hybrid Matching-aware Virtual Try-On Framework (HMaVTON), which combines retrieval-based and generative methods to foster a more personalized virtual try-on experience. This framework integrates a hybrid mix-and-match module and an enhanced virtual try-on module. The former can recommend fashion items available on the platform to boost sales and generate clothes that meets the diverse tastes of consumers. The latter provides high-quality try-on effects, delivering a one-stop shopping service. To validate the effectiveness of our approach, we enlist the expertise of fashion designers for a professional evaluation, assessing the rationality and diversity of the clothes combinations and conducting an evaluation matrix analysis. Our method significantly enhances the practicality of virtual try-on. The code is available at https://github.com/Yzcreator/HMaVTON.

==> sec/3_Method_before.tex <==
\section{Method}

Given a clothing-agnostic image $I \in \mathbb{R}^{3 \times H \times W}$ of a person, we propose the Generative Fashion Matching-aware Virtual Try-on Framework(GMVT). It extracts features from image $I$ and, through a diffusion process, generate matching cloth $I_0 \in \mathbb{R}^{3 \times H \times W}$ by incorporating external fashion knowledge. 
And this framework generates a visual representation $I_0^{'}  \in \mathbb{R}^{3 \times h \times w}$ of person wearing the generated clothing.


\subsection{Generative Matching Module(GMM)} \quad We design a method to introduce large-scale matching information in the try-on domain, addressing the issue of diminished model performance brought about by the scarcity of paired clothing items in try-on datasets. Simultaneously, we propose the Shape Constraint Network to obtain the shape constraints of matching clothing and use it together with the image $I$ as the guiding condition of the Matching Clothes Diffusion Network to generate matching clothing through denoising. The fusion of the shape constraints with visual cues ensures the generated matching clothing not only maintains its structural integrity but also achieves style coherence.


\subsubsection{Pre-train on External Matching Dataset} To address the issues of decreased model training accuracy and difficulty in creating innovative combinations due to sparse pairing data in the try-on dataset, we filter the clothing from the POG dataset~\cite{POG} and construct a large-scale matching clothing dataset. Within the Generative Matching Module, the Shape Constraint Network and the Matching Clothes Diffusion Network are trained on this dataset to learn ample matching knowledge. Subsequently, the pre-trained model undergoes fine-tuning on the try-on dataset, incorporating the learned matching information into the try-on domain. This enables the model to better capture the interrelationships and underlying patterns between clothing items, leading to an improved understanding of the ways in which clothing can be matched and the trends in fashion.

In the process of introducing matched information, the structural differences between the large-scale matching dataset and the try-on dataset's clothing pose a challenge. The large-scale matching dataset consists of flat-laid images featuring paired tops and bottoms, whereas the try-on dataset includes images of tops with models. This discrepancy makes it difficult for the model to transfer the learned matching information from the matching dataset to the try-on dataset. We adjust the clothing positions in the large matching dataset images to align with the training data in the try-on dataset. This allows the generative model to better learn the structure and features of the paired data.


 

\subsubsection{Shape Constraint Network} 
The image $I$ generates a matching clothing mask image $I_m  \in \mathbb{R}^{3 \times H \times W}$ through a shape-constrained network. These images are then separately used as inputs for VQ-GAN Encoder~\cite{esser2021taming} to obtain vectors. The two vectors are concatenated to form the external guiding condition vector $v_a$ for the diffusion model.


In our study, we utilize the U-Net network to predict the shape of clothing, and incorporate the resulting predictions as constraints in the denoising process. This approach enables the diffusion model to gain a better understanding of the image's structure and features, thereby mitigating the risk of erroneously identifying noise as valuable information during the denoising task. Furthermore, it enhances the model's robustness across different datasets and noise levels. During the training process, we employed the concept of GAN. The generator $G$ takes image $I$ as input and generates a matching clothing mask image $I_m$. The discriminator $D$ recognizes the output $I_m$ from the generator $G$ and accurately determines its authenticity. We employ a combination of cGAN~\cite{CGAN} loss and IoU~\cite{zhou2019iou} loss as the loss functions. This choice strikes a balance between preserving a certain level of structure and realism, while also emphasizing the similarity of the generated mask's shape to that of the ground truth mask:

\begin{equation}
    \mathcal{L}_{G}=\arg \min _G \max _D \mathcal{L}_{c G A N}(G, D)+\lambda \mathcal{L}_{IOU}(G).
\end{equation}



\subsubsection{Matching Clothes Diffusion Network} The image $I_T$, which is initialized with Gaussian noise for T steps, serves as the input. This module adopts the idea of ControlNet~\cite{zhang2023adding}, where during the training process, the model parameters of StableDiffusion~\cite{rombach2022high} are locked, and the parameters of its Encoder and Middle Block are simultaneously cloned as a trainable copy $ \Theta_c$. Define $\mathcal{Z}(\cdot ; \cdot)$ as the zero convolution operation, which is a 1x1 convolution layer with both weight and bias initialized to 0. And define $F( \cdot ; \cdot)$ as a neural network block operation, $\Theta_{z i}$ represents the parameters of the i-th zero convolution layer.

The external constraint vector $v_a$ is processed through a zero convolution to obtain $\mathcal{Z}\left(\boldsymbol{v_a} ; \Theta_{z 1}\right)$, and combined with the deep feature input $x$ through feature addition to yield $\boldsymbol{x}+\mathcal{Z}\left(\boldsymbol{v_a} ; \Theta_{z 1}\right)$. Further processing through block and zero convolution yields:

\begin{equation}
\mathcal{Z}\left(\mathcal{F}\left(\boldsymbol{x}+\mathcal{Z}\left(\boldsymbol{v_a} ; \Theta_{z 1}\right) ; \Theta_c\right) ; \Theta_{z 2}\right).
\end{equation}

This is subsequently combined with feature addition from the locked network to obtain the overall expression of image generation:

\begin{equation}
\boldsymbol{y}=\mathcal{F}(\boldsymbol{x} ; \Theta)+\mathcal{Z}\left(\mathcal{F}\left(\boldsymbol{x}+\mathcal{Z}\left(\boldsymbol{v_a} ; \Theta_{\mathrm{z} 1}\right) ; \Theta_{\mathrm{c}}\right) ; \Theta_{z 2}\right),
\end{equation} 
where $\Theta$ represents the locked parameters of the StableDiffusion model. Through the reverse denoising process, we obtain the generated matched clothing image $I_0$.  





\begin{figure*}
  \centering
  \includegraphics[width=1.0\textwidth]{image/result_matching.pdf}
  \caption{In comparison with baseline, our approach produces a diverse range of clothing styles, such as long sleeves, short sleeves, and straps, with color matching that adheres to the principles of harmony, creating a soothing visual resonance in terms of brightness and saturation.}
  \label{fig:result}
\end{figure*}



\subsection{Virtual Try-on Module(VTM)}
The module will dress the generated clothing on the character. Clothing and mask images generated from the GMM module, resized and combined with segmentation images from the dataset, serve as inputs to the Try-On Condition Generator to obtain warping clothes. The original image $I$, after Visual Fusion with warping clothes and denoising through a condition-guided diffusion model, produces the visualized try-on image.


\subsubsection{Try-On Condition Generator}  In this stage, we aim to obtain the clothing $\hat{W}$ that has been warped and deformed to align with the person's image. The Try-on condition generator operates based on the appearance flow deformation~\cite{lee2022high} and consists of two encoders, namely the clothing encoder $E_c$ and the segmentation encoder $E_s$. $E_c$ is used to extract features from clothing $I_c   \in \mathbb{R}^{3 \times h \times w}$ and mask $I_m \in \mathbb{L}^{h \times w}$, while $E_s$ extracts features from the segmentation map $I_d\in \mathbb{L}^{h \times w} $ and $I_p \in \mathbb{R}^{3 \times h \times w}$. Here, $\mathbb{L}$ represents semantic labels. The extracted features are fed into the flow pathway of the feature fusion block to generate the appearance flow map $F_{fi}$. It is then used to deform features extracted from $I_c$ and $I_m$, combining information from $E_c$ and $E_s$. Through feature alignment, warped cloth $\hat{W}_c$ and its corresponding mask $\hat{W}_m$, as well as the predicted segmentation map $I_s$, are obtained.

Try-on Condition Generator use $\mathcal{L}_{TV}$ to enhance the smoothness of the appearance flow:

\begin{equation}
    \mathcal {L}_{TV} = ||\nabla F_{f_4}||_1.
\end{equation}


L1 loss and perceptual loss are used to encourage the network to deform clothing to fit the pose of the person:



\begin{equation}
  \mathcal{L}_{L 1}=\sum_{i=0}^3 w_i \cdot\left\|D\left(I_m, F_{f_i}\right)-W_m\right\|_1+\left\|\hat{W}_m-W_m\right\|_1,
\end{equation}



\begin{equation}
    \mathcal{L}_{V G G}=\sum_{i=0}^3 w_i \cdot \phi\left(D\left(I_c, F_{f_i}\right), W_c\right)+\phi\left(\hat{W}_c, W_c\right),
\end{equation}
where $D(\cdot , \cdot)$ is defined as feature alignment, the operation involves removing non-overlapping regions. 
And $w_i$  represents the weight of relative importance.

In summary, Try-on Condition Generator is trained using the following loss function, where $\lambda_{L1}$, and $\lambda_{TV}$ represent hyperparameters controlling the relative importance between different losses:

\begin{equation}
    \mathcal{L}_{G}=\lambda_{L 1} \mathcal{L}_{L 1}+\mathcal{L}_{V G G}+\lambda_{T V} \mathcal{L}_{T V}.
\end{equation}




\subsubsection{Denoising Generator}
In Visual Fusion, we add the warped image $W_c$ to the original image $I$ and randomly introduce $T$ steps of Gaussian noise as the initial image $I_T^{'}$ for the diffusion model. The diffusion model loads fine-tuned Paint-by-Example parameters~\cite{DCI-VTON, yang2023paint},  and the generated clothing $I_c$ is encoded using the CLIP~\cite{CLIP} image encoder as a conditional input. This condition is injected into the network layers through cross-attention mechanism. Since the original information of the garment is contained in the image $I_T^{'}$, this facilitates the restoration of a more fitting wearing effect during the reverse diffusion process.




==> sec/other.tex <==

\begin{table*}
  \centering 
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline Index & Weights & Model & Very Satisfied & Satisfied & Average & Dissatisfied & Very Dissatisfied \\
    \hline \multirow{4}{*}{D1-Style Matching } & \multirow{4}{*}{$24 \%$} & FG & 0.070 & 0.300 & 0.388 & 0.182 & 0.06 \\
     & & Ours & 0.100 & 0.418 & 0.364 & 0.112 & 0.006 \\
     & & FR & 0.116 & 0.41 & 0.346 & 0.110 & 0.018 \\
     & & KFR & 0.122 & 0.456 & 0.314 & 0.090 & 0.018 \\
    \hline \multirow{4}{*}{D2-Color Matching } & \multirow{4}{*}{$25 \%$} & FG & 0.052 & 0.176 & 0.282 & 0.346 & 0.144 \\
     & & Ours & 0.090 & 0.348 & 0.346 & 0.200 & 0.016 \\
     & & FR & 0.120 & 0.376 & 0.330 & 0.152 & 0.022 \\
     & & KFR & 0.118 & 0.370 & 0.346 & 0.128 & 0.038 \\
    \hline \multirow{4}{*}{D3-Fabric Matching } & \multirow{4}{*}{$21 \%$} & FG & 54 & 0.224 & 0.344 & 0.296 & 0.082 \\
     & & Ours & 0.070 & 0.398 & 0.440 & 0.086 & 0.006 \\
     & & FR & 0.086 & 0.430 & 0.380 & 0.098 & 0.006 \\
     & & KFR & 0.128 & 0.460 & 0.322 & 0.078 & 0.012 \\
    \hline \multirow{4}{*}{D4-Variety } & \multirow{4}{*}{$30 \%$} & FG & 0.048 & 0.118 & 0.346 & 0.292 & 0.196 \\
     & & Ours & 0.076 & 0.420 & 0.390 & 0.106 & 0.008 \\
     & & FR & 0.128 & 0.400 & 0.370 & 0.086 & 0.016 \\
     & & KFR & 0.144 & 0.452 & 0.310 & 0.082 & 0.012 \\
    \hline
    \end{tabular}
  \caption{Weighted scoring of indicators}
  \label{tab:userstudy}
\end{table*}


\begin{table*}[h]
  \centering
  \begin{tabular}{c|ccccc|c}
    \toprule
    Model & Very Satisfied & Satisfied & Average & Dissatisfied & Very Dissatisfied & Overall Ratings\\
    \midrule
     FG & 0.056 & 0.198 & 0.340 & 0.280 & 0.126 & 2.777\\
     FR & 0.114 & 0.403 & 0.356 & 0.111 & 0.016 & 3.489\\
     KFR & 0.129 & 0.434 & 0.322 & 0.095 & 0.020 & 3.557\\
     Ours &  0.084 & 0.397 & 0.383 & 0.127 & 0.009 & 3.420\\
    \bottomrule
  \end{tabular}
  \caption{Try-on Results}
  \label{tab:satisfaction}
\end{table*}[h]


\section{Introduction}
ACM's consolidated article template, introduced in 2017, provides a
consistent \LaTeX\ style for use across ACM publications, and
incorporates accessibility and metadata-extraction functionality
necessary for future Digital Library endeavors. Numerous ACM and
SIG-specific \LaTeX\ templates have been examined, and their unique
features incorporated into this single new template.

If you are new to publishing with ACM, this document is a valuable
guide to the process of preparing your work for publication. If you
have published with ACM before, this document provides insight and
instruction into more recent changes to the article template.

The ``\verb|acmart|'' document class can be used to prepare articles
for any ACM publication --- conference or journal, and for any stage
of publication, from review to final ``camera-ready'' copy, to the
author's own version, with {\itshape very} few changes to the source.

\section{Template Overview}
As noted in the introduction, the ``\verb|acmart|'' document class can
be used to prepare many different kinds of documentation --- a
double-anonymous initial submission of a full-length technical paper, a
two-page SIGGRAPH Emerging Technologies abstract, a ``camera-ready''
journal article, a SIGCHI Extended Abstract, and more --- all by
selecting the appropriate {\itshape template style} and {\itshape
  template parameters}.

This document will explain the major features of the document
class. For further information, the {\itshape \LaTeX\ User's Guide} is
available from
\url{https://www.acm.org/publications/proceedings-template}.

\subsection{Template Styles}

The primary parameter given to the ``\verb|acmart|'' document class is
the {\itshape template style} which corresponds to the kind of publication
or SIG publishing the work. This parameter is enclosed in square
brackets and is a part of the {\verb|documentclass|} command:
\begin{verbatim}
  \documentclass[STYLE]{acmart}
\end{verbatim}

Journals use one of three template styles. All but three ACM journals
use the {\verb|acmsmall|} template style:
\begin{itemize}
\item {\texttt{acmsmall}}: The default journal template style.
\item {\texttt{acmlarge}}: Used by JOCCH and TAP.
\item {\texttt{acmtog}}: Used by TOG.
\end{itemize}

The majority of conference proceedings documentation will use the {\verb|acmconf|} template style.
\begin{itemize}
\item {\texttt{sigconf}}: The default proceedings template style.
\item{\texttt{sigchi}}: Used for SIGCHI conference articles.
\item{\texttt{sigplan}}: Used for SIGPLAN conference articles.
\end{itemize}

\subsection{Template Parameters}

In addition to specifying the {\itshape template style} to be used in
formatting your work, there are a number of {\itshape template parameters}
which modify some part of the applied template style. A complete list
of these parameters can be found in the {\itshape \LaTeX\ User's Guide.}

Frequently-used parameters, or combinations of parameters, include:
\begin{itemize}
\item {\texttt{anonymous,review}}: Suitable for a ``double-anonymous''
  conference submission. Anonymizes the work and includes line
  numbers. Use with the \texttt{\acmSubmissionID} command to print the
  submission's unique ID on each page of the work.
\item{\texttt{authorversion}}: Produces a version of the work suitable
  for posting by the author.
\item{\texttt{screen}}: Produces colored hyperlinks.
\end{itemize}

This document uses the following string as the first command in the
source file:
\begin{verbatim}
\documentclass[sigconf]{acmart}
\end{verbatim}

\section{Modifications}

Modifying the template --- including but not limited to: adjusting
margins, typeface sizes, line spacing, paragraph and list definitions,
and the use of the \verb|\vspace| command to manually adjust the
vertical spacing between elements of your work --- is not allowed.

{\bfseries Your document will be returned to you for revision if
  modifications are discovered.}

\section{Typefaces}

The ``\verb|acmart|'' document class requires the use of the
``Libertine'' typeface family. Your \TeX\ installation should include
this set of packages. Please do not substitute other typefaces. The
``\verb|lmodern|'' and ``\verb|ltimes|'' packages should not be used,
as they will override the built-in typeface families.

\section{Title Information}

The title of your work should use capital letters appropriately -
\url{https://capitalizemytitle.com/} has useful rules for
capitalization. Use the {\verb|title|} command to define the title of
your work. If your work has a subtitle, define it with the
{\verb|subtitle|} command.  Do not insert line breaks in your title.

If your title is lengthy, you must define a short version to be used
in the page headers, to prevent overlapping text. The \verb|title|
command has a ``short title'' parameter:
\begin{verbatim}
  \title[short title]{full title}
\end{verbatim}

\section{Authors and Affiliations}

Each author must be defined separately for accurate metadata
identification.  As an exception, multiple authors may share one
affiliation. Authors' names should not be abbreviated; use full first
names wherever possible. Include authors' e-mail addresses whenever
possible.

Grouping authors' names or e-mail addresses, or providing an ``e-mail
alias,'' as shown below, is not acceptable:
\begin{verbatim}
  \author{Brooke Aster, David Mehldau}
  \email{dave,judy,steve@university.edu}
  \email{firstname.lastname@phillips.org}
\end{verbatim}

The \verb|authornote| and \verb|authornotemark| commands allow a note
to apply to multiple authors --- for example, if the first two authors
of an article contributed equally to the work.

If your author list is lengthy, you must define a shortened version of
the list of authors to be used in the page headers, to prevent
overlapping text. The following command should be placed just after
the last \verb|\author{}| definition:
\begin{verbatim}
  \renewcommand{\shortauthors}{McCartney, et al.}
\end{verbatim}
Omitting this command will force the use of a concatenated list of all
of the authors' names, which may result in overlapping text in the
page headers.

The article template's documentation, available at
\url{https://www.acm.org/publications/proceedings-template}, has a
complete explanation of these commands and tips for their effective
use.

Note that authors' addresses are mandatory for journal articles.

\section{Rights Information}

Authors of any work published by ACM will need to complete a rights
form. Depending on the kind of work, and the rights management choice
made by the author, this may be copyright transfer, permission,
license, or an OA (open access) agreement.

Regardless of the rights management choice, the author will receive a
copy of the completed rights form once it has been submitted. This
form contains \LaTeX\ commands that must be copied into the source
document. When the document source is compiled, these commands and
their parameters add formatted text to several areas of the final
document:
\begin{itemize}
\item the ``ACM Reference Format'' text on the first page.
\item the ``rights management'' text on the first page.
\item the conference information in the page header(s).
\end{itemize}

Rights information is unique to the work; if you are preparing several
works for an event, make sure to use the correct set of commands with
each of the works.

The ACM Reference Format text is required for all articles over one
page in length, and is optional for one-page articles (abstracts).

\section{CCS Concepts and User-Defined Keywords}

Two elements of the ``acmart'' document class provide powerful
taxonomic tools for you to help readers find your work in an online
search.

The ACM Computing Classification System ---
\url{https://www.acm.org/publications/class-2012} --- is a set of
classifiers and concepts that describe the computing
discipline. Authors can select entries from this classification
system, via \url{https://dl.acm.org/ccs/ccs.cfm}, and generate the
commands to be included in the \LaTeX\ source.

User-defined keywords are a comma-separated list of words and phrases
of the authors' choosing, providing a more flexible way of describing
the research being presented.

CCS concepts and user-defined keywords are required for for all
articles over two pages in length, and are optional for one- and
two-page articles (or abstracts).

\section{Sectioning Commands}

Your work should use standard \LaTeX\ sectioning commands:
\verb|section|, \verb|subsection|, \verb|subsubsection|, and
\verb|paragraph|. They should be numbered; do not remove the numbering
from the commands.

Simulating a sectioning command by setting the first word or words of
a paragraph in boldface or italicized text is {\bfseries not allowed.}

\section{Tables}

The ``\verb|acmart|'' document class includes the ``\verb|booktabs|''
package --- \url{https://ctan.org/pkg/booktabs} --- for preparing
high-quality tables.

Table captions are placed {\itshape above} the table.

Because tables cannot be split across pages, the best placement for
them is typically the top of the page nearest their initial cite.  To
ensure this proper ``floating'' placement of tables, use the
environment \textbf{table} to enclose the table's contents and the
table caption.  The contents of the table itself must go in the
\textbf{tabular} environment, to be aligned properly in rows and
columns, with the desired horizontal and vertical rules.  Again,
detailed instructions on \textbf{tabular} material are found in the
\textit{\LaTeX\ User's Guide}.

Immediately following this sentence is the point at which
Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed output of
this document.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

To set a wider table, which takes up the whole width of the page's
live area, use the environment \textbf{table*} to enclose the table's
contents and the table caption.  As with a single-column table, this
wide table will ``float'' to a location deemed more
desirable. Immediately following this sentence is the point at which
Table~\ref{tab:commands} is included in the input file; again, it is
instructive to compare the placement of the table here with the table
in the printed output of this document.

\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}

Always use midrule to separate table header rows from data rows, and
use it only for this purpose. This enables assistive technologies to
recognise table headers and support their users in navigating tables
more easily.

\section{Math Equations}
You may want to display math equations in three distinct styles:
inline, numbered or non-numbered display.  Each of the three are
discussed in the next sections.

\subsection{Inline (In-text) Equations}
A formula that appears in the running text is called an inline or
in-text formula.  It is produced by the \textbf{math} environment,
which can be invoked with the usual
\texttt{{\char'134}begin\,\ldots{\char'134}end} construction or with
the short form \texttt{\$\,\ldots\$}. You can use any of the symbols
and structures, from $\alpha$ to $\omega$, available in
\LaTeX~\cite{Lamport:LaTeX}; this section will simply show a few
examples of in-text equations in context. Notice how this equation:
\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\subsection{Display Equations}
A numbered display equation---one set off by vertical space from the
text and centered horizontally---is produced by the \textbf{equation}
environment. An unnumbered display equation is produced by the
\textbf{displaymath} environment.

Again, in either environment, you can use any of the symbols and
structures available in \LaTeX\@; this section will just give a couple
of examples of display equations in context.  First, consider the
equation, shown as an inline equation above:
\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}
Notice how it is formatted somewhat differently in
the \textbf{displaymath}
environment.  Now, we'll enter an unnumbered equation:
\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}
and follow it with another numbered equation:
\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}
just to demonstrate \LaTeX's able handling of numbering.

\section{Figures}

The ``\verb|figure|'' environment should be used for figures. One or
more images can be placed within a figure. If your figure contains
third-party material, you must clearly identify it as such, as shown
in the example below.
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{sample-franklin}
  \caption{1907 Franklin Model D roadster. Photograph by Harris \&
    Ewing, Inc. [Public domain], via Wikimedia
    Commons. (\url{https://goo.gl/VLCRBB}).}
  \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}

Your figures should contain a caption which describes the figure to
the reader.

Figure captions are placed {\itshape below} the figure.

Every figure should also have a figure description unless it is purely
decorative. These descriptions convey what’s in the image to someone
who cannot see it. They are also used by search engine crawlers for
indexing images, and when images cannot be loaded.

A figure description must be unformatted plain text less than 2000
characters long (including spaces).  {\bfseries Figure descriptions
  should not repeat the figure caption – their purpose is to capture
  important information that is not already provided in the caption or
  the main text of the paper.} For figures that convey important and
complex new information, a short text description may not be
adequate. More complex alternative descriptions can be placed in an
appendix and referenced in a short figure description. For example,
provide a data table capturing the information in a bar chart, or a
structured list representing a graph.  For additional information
regarding how best to write figure descriptions and why doing this is
so important, please see
\url{https://www.acm.org/publications/taps/describing-figures/}.

\subsection{The ``Teaser Figure''}

A ``teaser figure'' is an image, or set of images in one figure, that
are placed after all author and affiliation information, and before
the body of the article, spanning the page. If you wish to have such a
figure in your article, place the command immediately before the
\verb|\maketitle| command:
\begin{verbatim}
  \begin{teaserfigure}
    \includegraphics[width=\textwidth]{sampleteaser}
    \caption{figure caption}
    \Description{figure description}
  \end{teaserfigure}
\end{verbatim}

\section{Citations and Bibliographies}

The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

The bibliography is included in your source document with these two
commands, placed just before the \verb|\end{document}| command:
\begin{verbatim}
  \bibliographystyle{ACM-Reference-Format}
  \bibliography{bibfile}
\end{verbatim}
where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
suffix, of the \BibTeX\ file.

Citations and references are numbered by default. A small number of
ACM publications have citations and references formatted in the
``author year'' style; for these exceptions, please include this
command in the {\bfseries preamble} (before the command
``\verb|\begin{document}|'') of your \LaTeX\ source:
\begin{verbatim}
  \citestyle{acmauthoryear}
\end{verbatim}


  Some examples.  A paginated journal article \cite{Abril07}, an
  enumerated journal article \cite{Cohen07}, a reference to an entire
  issue \cite{JCohen96}, a monograph (whole book) \cite{Kosiur01}, a
  monograph/whole book in a series (see 2a in spec. document)
  \cite{Harel79}, a divisible-book such as an anthology or compilation
  \cite{Editor00} followed by the same example, however we only output
  the series if the volume number is given \cite{Editor00a} (so
  Editor00a's series should NOT be present since it has no vol. no.),
  a chapter in a divisible book \cite{Spector90}, a chapter in a
  divisible book in a series \cite{Douglass98}, a multi-volume work as
  book \cite{Knuth97}, a couple of articles in a proceedings (of a
  conference, symposium, workshop for example) (paginated proceedings
  article) \cite{Andler79, Hagerup1993}, a proceedings article with
  all possible elements \cite{Smith10}, an example of an enumerated
  proceedings article \cite{VanGundy07}, an informally published work
  \cite{Harel78}, a couple of preprints \cite{Bornmann2019,
    AnzarootPBM14}, a doctoral dissertation \cite{Clarkson85}, a
  master's thesis: \cite{anisi03}, an online document / world wide web
  resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game
  (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03} and \cite{Lee05}
  and (Case 3) a patent \cite{JoeScientist001}, work accepted for
  publication \cite{rous08}, 'YYYYb'-test for prolific author
  \cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might
  contain 'duplicate' DOI and URLs (some SIAM articles)
  \cite{Kirschmer:2010:AEI:1958016.1958018}. Boris / Barbara Beeton:
  multi-volume works as books \cite{MR781536} and \cite{MR781537}. A
  couple of citations with DOIs:
  \cite{2004:ITE:1009386.1010128,Kirschmer:2010:AEI:1958016.1958018}. Online
  citations: \cite{TUGInstmem, Thornburg01, CTANacmart}.
  Artifacts: \cite{R} and \cite{UMassCitations}.

\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

\section{Appendices}

If your work needs an appendix, add it before the
``\verb|\end{document}|'' command at the conclusion of your source
document.

Start the appendix with the ``\verb|appendix|'' command:
\begin{verbatim}
  \appendix
\end{verbatim}
and note that in the appendix, sections are lettered, not
numbered. This document has two appendices, demonstrating the section
and subsection identification method.

\section{Multi-language papers}

Papers may be written in languages other than English or include
titles, subtitles, keywords and abstracts in different languages (as a
rule, a paper in a language other than English should include an
English title and an English abstract).  Use \verb|language=...| for
every language used in the paper.  The last language indicated is the
main language of the paper.  For example, a French paper with
additional titles and abstracts in English and German may start with
the following command
\begin{verbatim}
\documentclass[sigconf, language=english, language=german,
               language=french]{acmart}
\end{verbatim}

The title, subtitle, keywords and abstract will be typeset in the main
language of the paper.  The commands \verb|\translatedXXX|, \verb|XXX|
begin title, subtitle and keywords, can be used to set these elements
in the other languages.  The environment \verb|translatedabstract| is
used to set the translation of the abstract.  These commands and
environment have a mandatory first argument: the language of the
second argument.  See \verb|sample-sigconf-i13n.tex| file for examples
of their usage.

\section{SIGCHI Extended Abstracts}

The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
not in Word) produces a landscape-orientation formatted article, with
a wide left margin. Three environments are available for use with the
``\verb|sigchi-a|'' template style, and produce formatted output in
the margin:
\begin{description}
\item[\texttt{sidebar}:]  Place formatted text in the margin.
\item[\texttt{marginfigure}:] Place a figure in the margin.
\item[\texttt{margintable}:] Place a table in the margin.
\end{description}

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
\begin{acks}
To Robert, for the bagels and explaining CMYK and color spaces.
\end{acks}




\begin{table*}
  \centering 
  \caption{Results of Clothing Design Expert Evaluation. Our model's scores closely align with retrieval-based models, indicating that our outcomes not only offer users more diverse options but also provide fashion designers with a broader spectrum of design inspiration.}
  \setlength{\abovecaptionskip}{0.0cm}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \hline Model & Index & Weight & Very Satisfied & Satisfied & Average & Dissatisfied & Very Dissatisfied & Score \\
    \hline \multirow{5}{*}{GenMatching} & D1-Style & $24 \%$ & 0.070 & 0.300 & 0.388 & 0.182 & 0.06 & \multirow{5}{*}{2.777}\\
     &D2-Color & $25 \%$ & 0.052 & 0.176 & 0.282 & 0.346 & 0.144  \\
     &D3-Fabric & $21 \%$ & 0.054 & 0.224 & 0.344 & 0.296 & 0.082 \\
     &D4-Variety& $30 \%$ & 0.048 & 0.118 & 0.346 & 0.292 & 0.196 \\
     &Average & - & 0.056 & 0.198 & \textbf{0.340} & 0.280 & 0.126 \\
     
    \hline \multirow{5}{*}{RetMatching} & D1-Style & $24 \%$ & 0.116 & 0.41 & 0.346 & 0.110 & 0.018 & \multirow{5}{*}{3.489}\\
     &D2-Color & $25 \%$ & 0.120 & 0.376 & 0.330 & 0.152 & 0.022 \\
     &D3-Fabric & $21 \%$ & 0.086 & 0.430 & 0.380 & 0.098 & 0.006 \\
     &D4-Variety& $30 \%$ & 0.144 & 0.452 & 0.310 & 0.082 & 0.012 \\
     &Average & - & 0.114 & \textbf{0.403} & 0.356 & 0.111 & 0.016 \\
     
    \hline \multirow{5}{*}{\begin{tabular}{c}
         RetMatching+\\
    \end{tabular}} & D1-Style & $24 \%$ & 0.122 & 0.456 & 0.314 & 0.090 & 0.018 & \multirow{5}{*}{3.557}\\
     &D2-Color & $25 \%$ & 0.118 & 0.370 & 0.346 & 0.128 & 0.038 \\
     &D3-Fabric & $21 \%$ & 0.128 & 0.460 & 0.322 & 0.078 & 0.012 \\
     &D4-Variety& $30 \%$ & 0.144 & 0.452 & 0.310 & 0.082 & 0.012 \\
     &Average & - & 0.129 & \textbf{0.434} & 0.322 & 0.095 & 0.020 \\
     
    \hline \multirow{5}{*}{\begin{tabular}{c}
         \textbf{GMVT(Ours)}
    \end{tabular}} & D1-Style & $24 \%$ & 0.100 & 0.418 & 0.364 & 0.112 & 0.006 & \multirow{5}{*}{3.420}\\
     &D2-Color & $25 \%$ & 0.090 & 0.348 & 0.346 & 0.200 & 0.016 \\
     &D3-Fabric & $21 \%$ & 0.070 & 0.398 & 0.440 & 0.086 & 0.006 \\
     &D4-Variety& $30 \%$ & 0.076 & 0.420 & 0.390 & 0.106 & 0.008 \\
     &Average & - & 0.084 & \textbf{0.397} & 0.383 & 0.127 & 0.009 \\
    \hline
    \end{tabular}


  \label{tab:userstudy}
\end{table*}





To comprehensively evaluate the performance of virtual try-on, we utilized a variety of widely recognized quantitative analysis metrics for detailed testing and analysis. Specifically, we employed the Structural Similarity Index (SSIM)~\cite{wang2004image} to measure the similarity between generated images and real images in aspects such as brightness, contrast, and structural information. Furthermore, we used the Fréchet Inception Distance (FID) ~\cite{parmar2022aliased} to assess the distance between generated and real images in feature space, thus quantifying the quality of the generated images. The Kernel Inception Distance (KID) ~\cite{binkowski2018demystifying} was applied to gauge the discrepancy between the real and generated distributions, capturing more subtle statistical characteristics using kernel methods. Additionally, we implemented the Inception Score (IS) ~\cite{barratt2018note} to evaluate the clarity and diversity of the generated images. Perceptually, the Learned Perceptual Image Patch Similarity (LPIPS) ~\cite{zhang2018unreasonable} evaluated the visual differences between images, which, unlike traditional pixel-level differences, is closer to human visual perception. The Peak Signal-to-Noise Ratio (PSNR) ~\cite{hore2010image} was used to measure the quality of image reconstruction, assessing the fidelity of generated images relative to the originals. To further validate the effectiveness of the Shape Constraint Network, we employed not only the above metrics but also introduced the YOLOScore ~\cite{li2021image} as an evaluation criterion. Through these in-depth and multi-faceted quantitative metrics, we were able to meticulously assess the comprehensive performance of Matching-aware Generation and virtual try-on technology, thereby ensuring that the proposed system meets the users' demands for high quality and precision.





We design a method to introduce large-scale matching information in the try-on domain, addressing the issue of diminished model performance brought about by the scarcity of paired clothing items in try-on datasets. 




